Signaling in Bayesian Network Congestion Games: the Subtle Power of Symmetry

Network congestion games are a well-understood model of multi-agent strategic interactions. Despite their ubiquitous applications, it is not clear whether it is possible to design information structures to ameliorate the overall experience of the network users. We focus on Bayesian games with atomic players, where network vagaries are modeled via a (random) state of nature which determines the costs incurred by the players. A third-party entity---the sender---can observe the realized state of the network and exploit this additional information to send a signal to each player. A natural question is the following: is it possible for an informed sender to reduce the overall social cost via the strategic provision of information to players who update their beliefs rationally? The paper focuses on the problem of computing optimal ex ante persuasive signaling schemes, showing that symmetry is a crucial property for its solution. Indeed, we show that an optimal ex ante persuasive signaling scheme can be computed in polynomial time when players are symmetric and have affine cost functions. Moreover, the problem becomes NP-hard when players are asymmetric, even in non-Bayesian settings.

==> prelim.tex <==
\section{Preliminaries}\label{sec:prelim}

We study non-atomic network congestion games in which the edge costs depend on a stochastic state of nature. 
%
We tackle this scenario using the model of Bayesian persuasion introduced by~\citet{kamenica2011bayesian}, \emph{i.e.}, we assume that there is a \emph{sender} who can observe the state of nature and, based on that, privately communicate signals to the players (acting as \emph{receivers}) in such a way to persuade them to follow the desired routes in the network.
\todoac{Secondo me dovremmo spiegare meglio che senso ha il framework BP in questo setting. Non si capisce da dove salti fuori {\em sender} etc.}

A \emph{network congestion game} (NCG) is defined as a tuple $(N,G,\{c_e\}_{e \in E},\{(s_p,t_p)\}_{p \in N})$, where:
%
$N = \{1, \ldots, n\}$ denotes the set of players;

\todoac{Se $N$ diventasse $\mathcal{P}$? Non mi piace $p\in N$.}
\todoac{$\mathbb{Q}\to \mathbb{R}$}

%
$G = (V,E)$ is the directed graph underlying the game, with $V$ being its set of nodes and each $e = (v,v') \in E$ representing a directed edge from $v$ to $v'$;
%
$\{c_e\}_{e \in E}$ are the edge costs, with each $c_e : \mathbb{N} \to \mathbb{Q}_+$ defining the cost of edge $e \in E$ as a function of the number of players traveling through $e$;
%
finally, $\{(s_p,t_p)\}_{p \in N}$, with $s_p, t_p \in V$, denote the source-destination pairs for all the players.
%
As usual, we assume that $c_e(0) = 0$ for all $e \in E$.

In a NCG, the set $A_p$ of actions available to a player $p \in N$ is implicitly defined by the graph $G$, the source $s_p$, and the destination $t_p$.
%
Formally, $A_p$ is the set of all directed paths from $s_p$ to $t_p$ in the graph $G$.
%
In this work, we use $a_p \in A_p$ to denote a player $p$'s path and we write $e \in a_p$ whenever the path contains the edge $e \in E$.
%
An action profile $a \in A$, where $A = \bigtimes_{p \in N} A_p$, is a tuple of $s_p$-$t_p$ directed paths $a_p \in A_p$, one per player $p \in N$.
%
For the ease of notation, given an action profile $a \in A$, we let $f_e^a$ be the congestion of edge $e \in E$ in $a$, \emph{i.e.}, the number of players selecting a path passing thorough $e$ in $a$; formally, $f_e^a = |\{ p \in N \mid e \in a_p  \}|$.
%
Thus, $c_e(f_e^a)$ denotes the cost of edge $e$ in $a$.
%
Finally, we let the cost incurred by player $p \in N$ in an action profile $a \in A$ be denoted as $c_p(a) = \sum_{e \in a_p} c_e(f_e^a)$.

\todoac{Ref per BNCG?}
We define a \emph{Bayesian network congestion game} (BNCG) as a tuple $(N,G,\Theta, \mu, \{c_{e,\theta}\}_{e \in E, \theta \in \Theta},\{(s_p,t_p)\}_{p \in N})$, where, differently from the basic setting, the edge cost functions $c_{e,\theta}: \mathbb{N} \to \mathbb{Q}_+$ also depend on a state of nature $\theta$ drawn from a finite set of states $\theta$.
%
Moreover, $\mu$ encodes the prior beliefs that the players have over the states of nature $\Theta$, \emph{i.e.}, $\mu \in \textnormal{int}(\Delta_\Theta)$ is a fully-supported probability distribution over the set $\Theta$, with $\mu_\theta$ denoting the prior probability that the state of nature is $\theta \in \Theta$.
%
All the other components are defined as in non-Bayesian NCGs.
%
Notice that, in BNCGs, the cost experienced by player $p \in N$ in an action profile $a \in A$ also depends on the state of nature $\theta \in \Theta$, and, thus, it is defined as $c_{p,\theta}(a) = \sum_{e \in a_p} c_{e,\theta}(f_e^a)$.

In this work, we will focus on BNCGs with two additional properties.
%
First, we say that a BNCG is \emph{symmetric} if all the players share the same $s_p$-$t_p$ pair, \emph{i.e.}, whenever they all have the same set of actions (paths) available.
%
For the ease of notation, in such settings we let $s, t \in V$ be the common source and destination.
%
Moreover, a BNCG has \emph{affine costs} if the edge cost functions are affine in the edge congestion, \emph{i.e.}, for all $e \in E$ and $\theta \in \Theta$, there exist constants $\alpha_{e,\theta}, \beta_{e,\theta} \in \mathbb{Q}_+$ such that we can write $c_{e,\theta}(f_e^a) = \alpha_{e,\theta} f_e^a + \beta_{e,\theta}$.
\todoac{Perche' a qualcuno dovrebbe fregare qualcosa di BNCG simmetriche e affini? :) }
\todoac{Esempio qui? (con ottimo misto?)}
